Learnt Sparsification for Interpretable Graph Neural Networks

Graph neural networks (GNNs) have achieved great success on various tasks and fields that require relational modeling. GNNs aggregate node features using the graph structure as inductive biases resulting in flexible and powerful models. However, GNNs remain hard to interpret as the interplay between node features and graph structure is only implicitly learned. In this paper, we propose a novel method called Kedge for explicitly sparsifying the underlying graph by removing unnecessary neighbors. Our key idea is based on a tractable method for sparsification using the Hard Kumaraswamy distribution that can be used in conjugation with any GNN model. Kedge learns edge masks in a modular fashion trained with any GNN allowing for gradient based optimization in an end-to-end fashion. We demonstrate through extensive experiments that our model Kedge can prune a large proportion of the edges with only a minor effect on the test accuracy. Specifically, in the PubMed dataset, Kedge learns to drop more than 80% of the edges with an accuracy drop of merely 2% showing that graph structure has only a small contribution in comparison to node features. Finally, we also show that Kedge effectively counters the over-smoothing phenomena in deep GNNs by maintaining good task performance with increasing GNN layers.

==> 04_problem.tex <==
\section{HardKuma Distribution}
\label{sec:HardKuma}
\todo[inline]{I would suggest to introduce Hard Kuma as  areparamey}
 The main idea in our work is to learn the probability distribution over the edges in the graph to drop the task irrelevant edges. For this we used a Hard Kumaraswamy (in short HardKuma) distribution, introduced by ~\cite{bastings2019interpretable}, that exhibits both continuous and discrete behaviour. This distribution can learn to sample exactly 0 or exactly 1 and this learning process is differentiable.
 
 %Overall, We can start from the distribution over open interval (0,1)(blue dashed curve in figure \ref{fig1}) and can stretch the support from \textit{l to r} where $l<0$ and $r>1$ to include \{0\} and \{1\}. Finally we can integrate the masses over semi-open intervals (\textit{l},0] and [1,r) to \{0\} and \{1\} respectively (red shaded areas in fig.\ref{fig1}). as described in equations (\ref{6}) and (\ref{7}).
% We used the Hard Kumaraswamy distribution introduced by \cite{bastings2019interpretable}. In which they used this \textit{stretch-and-rectify} technique over Kumaraswamy distribution\cite{kumaraswamy1980generalized} which is similar to \textit{Beta} distribution. This \textit{stretch-and-rectify} technique was introduced by \cite{louizos2017learning} in which they rectified samples from the BinaryConcrete (or GumbelSoftmax).  distribution\cite{maddison2016concrete}\cite{jang2017categorical}


% In which they used this \textit{stretch-and-rectify} technique over Kumaraswamy distribution\cite{kumaraswamy1980generalized} which is similar to \textit{Beta} distribution. This \textit{stretch-and-rectify} technique was introduced by \cite{louizos2017learning} in which they rectified samples from the BinaryConcrete (or GumbelSoftmax).  distribution\cite{maddison2016concrete}\cite{jang2017categorical}


\subsection{Kuma and HardKuma Distributions}

The HardKuma is an extension of Kumaraswamy (Kuma) distribution~\cite{kumaraswamy1980generalized}. We will start with defining the Kuma distribution.
Fig.~\ref{fig:kuma} shows the relations between the probability density function (PDF) of Kuma and Stretched Kuma distribution. 


\begin{figure}
  \centering
  \includegraphics[width=8cm]{hardkuma_labl.png}
  \caption{On x-axis, we have support for the distributions. Kuma(0.5,0.5) (blue dashed line) is the PDF for Kuma distribution with support (0,1) and StretchedKuma(0.5,0.5,-0.1,1.1)(red line) is the PDF of Stretched Kuma with support (-0.1,1.1). The red region formed by integrating the mass of (-0.1,0] to \{0\} and [1,1.1) to \{1\}.
    }
  \label{fig:kuma}
\end{figure}

\begin{definition}[Kuma Distribution]
A random variable Y is said to be have a Kuma distribution if its PDF is given by
\begin{equation}
 f_{Y}(y ; \alpha, \beta)=\alpha \beta y^{\alpha-1}\left(1-y^{\alpha}\right)^{\beta-1}, \quad y \in(0,1)
\end{equation}
where $\alpha, \beta > 0$ and has the following cumulative distribution function (CDF)
\begin{equation}
F_{Y}(y ; \alpha, \beta)=1-\left(1-y^{\alpha}\right)^{\beta}.
\end{equation}
\end{definition}

The support of the original Kuma distribution doesn't include 0 and 1.
Hence, we define the Stretched Kuma distribution, which has the support $(l,r)$. 

\begin{definition}[Stretched Kuma Distribution]
Let $F_{Y}(y ; \alpha, \beta)$ be the CDF of the Kuma distributed random variable $Y\sim \operatorname{Kuma}(\alpha,\beta)$. A random variable T is said to have a Stretched Kuma distribution with support $(l,r)$ if its CDF is given by
\begin{equation}
F_{T}(t ; \alpha, \beta,l,r)= F_{Y}\left(\frac{t-l}{r-l}; \alpha, \beta\right), \quad t\in (l,r).
\end{equation}
 where $l<0$ and $r>1$ and PDF is given by
\begin{equation}
 f_{T}(t ; \alpha, \beta, l, r)=f_{Y}\left(\frac{t-l}{r-l} ; \alpha, \beta \right) \frac{1}{(r-l)}
\end{equation}
where $r-l>0$.
\end{definition}

To retrieve HardKuma distributions, we sample a point $t$ from the Stretched Kuma distribution and apply hard sigmoid, i.e.,  $h = \min(1, \max(0, t))$, afterwards. 
As shown in Fig.~\ref{fig:kuma}, the likelihood for sampling 0 is equal to sampling any point $t < 0$ for the underlying Stretched Kuma. Similarly the likelihood of a $1$ is equivalent to sampling $t>1$.
Hence the probability at $h=0$ and $h=1$ is defined in closed form.
\begin{definition}[HardKuma Distribution~\cite{bastings2019interpretable}]
Let $\alpha, \beta >0$, $l<0$, and $r>1$. Then the PDF of a HardKuma distribution is given by
\begin{equation}
    f_{HK}(h; \alpha, \beta, l, r) = 
    \begin{cases}
    F_{Y}\left(\frac{-l}{r-l} ; \alpha, \beta\right), &\text{ for } h=0,\\
    1-F_{Y}\left(\frac{1-l}{r-l} ; \alpha, \beta\right), &\text{ for } h=1,\\
     f_{T}(h ; \alpha, \beta, l, r) &\text{ for } h\in (0,1).
    \end{cases}
\end{equation}
\end{definition}

The reasons for selecting HardKuma distribution for our \approach{} are the following: 

\mpara{Properties of HardKuma.}
The HardKuma distribution with parameters $\alpha, \beta, l, r$ has the following properties
\begin{enumerate}
    \item Having 0 and 1 in the support of HardKuma distribution, It is possible to sample exactly 0 or exactly 1 using HardKuma distribution with \textit{non-zero} probability.
    \item The reparameterization is differentiable. 

\end{enumerate}

%To get samples from HardKuma, we start with sampling from Kuma distribution. Since inverse of kuma CDF is in closed form and eq.(\ref{eq:10}) holds, We used \textit{inverse CDF} method to get samples from Kuma distribution. So, fist we apply inverse CDF of Kuma distribution($Y \sim \texttt{Kuma}(\alpha, \beta)$) over $U\sim \mathcal{U}(0, 1)$ as eq.(\ref{eq:10a}), then shifting and scaling the result to cover the stretched support (eq.\ref{eq:10b}), and finally rectify using \textit{hard-sigmoid} in order to get the sample in the closed interval [0, 1] (eq.\ref{eq:10c}).
%\thorben{in any case you should use a continous way of referencing equations. I prefer, e.g. Eq. (1), but you can also use eqref, e.g. \eqref{eq:10} }
 
%\begin{equation}
%F_{Y}^{-1}(U ; \alpha, \beta) \sim \operatorname{Kuma}(\alpha, \beta)
%\label{eq:10}
%\end{equation}

%\begin{equation}
 %   y=F_{Y}^{-1}(u ; \alpha, \beta)=\left(1-(1-u)^{1 / \beta}\right)^{1/\alpha}
 %   \label{eq:10a}
%\end{equation}    
%\begin{equation}
 %       t=l+(r-l)y
  %      \label{eq:10b}
%\end{equation}
%\begin{equation}
 %       h=\min (1, \max (0, t))
  %      \label{eq:10c}
%\end{equation}
%We defined the probabilities for sampling exactly 0 or exactly 1 in definition of HardKuma.

%%%%%%%%%%%%%%%  
  
% Let $H\sim \texttt{HardKuma}(\alpha, \beta, l, r)$ be a rectified random variable defined by passing a sample $T\sim\texttt{Kuma}(\alpha, \beta, l, r)$ through hard sigmoid, i.e.  $h = \texttt{min}(1, \texttt{max}(0, t))$. The $H\sim \texttt{HardKuma}(\alpha, \beta, l, r)$ is now defined on closed interval [0,1]. 
% 
% If 0 is the probability of
% sampling t=0, note that sampling h=0 is equivalent to sample any $t_0\in(l,0]$. 
% 
% Similarly, with 0 probability of
% sampling t=1, sampling h=1 is equivalent to sample any $t_1\in[1,r)$. Hence $\forall t_0 \in (\textit{l},0]$ and $\forall  t_1 \in [1, r)$, is deterministically mapped to 0 and 1 respectively(see red region in fig.\ref{fig2}), hence the probability at h=0 and h=1 is defined in closed form as following: 

% \begin{equation}
%     \mathbb{P}(H=0)=F_{Y}\left(\frac{-l}{r-l} ; \alpha, \beta\right),
%     \label{6}
% \end{equation}
% \begin{equation}
%     \mathbb{P}(H=1)=1-F_{Y}\left(\frac{1-l}{r-l} ; \alpha, \beta\right)
%     \label{7}
% \end{equation}
% and 
% \begin{equation}
%     \mathbb{P}(0<H<1)=1-\mathbb{P}(H=0)-\mathbb{P}(H=1)
% \end{equation}




\subsection{Sampling from HardKuma and Gradients} 
We cannot directly sample points from HardKuma distribution. 
To get samples from HardKuma, we need samples from Kuma distribution. Since inverse of Kuma CDF is in closed form, we use \textit{inverse CDF} method to get samples from Kuma distribution. 
Hence, we start by sampling $u$ from uniform distribution from $U\sim \mathcal{U}(0, 1)$. Then we apply inverse CDF of Kuma distribution to $u$ and retrieve a sample from $Y\sim \operatorname{Kuma}(\alpha, \beta)$.
Then shifting and scaling the result to cover the stretched support $(l, r)$. 
Finally rectify using \textit{hard-sigmoid} in order to get the sample in the closed interval $[0, 1]$.
\begin{equation}
    z=\mathtt{HardKuma}(u,\alpha,\beta,l,r)
\end{equation}
We defined the probabilities for sampling exactly 0 or exactly 1 in definition of HardKuma.


%\begin{equation}
%F_{Y}^{-1}(U ; \alpha, \beta) \sim \operatorname{Kuma}(\alpha, \beta)
%\label{eq:10}
%\end{equation}

%\begin{equation}
 %   y=F_{Y}^{-1}(u ; \alpha, \beta)=\left(1-(1-u)^{1 / \beta}\right)^{1/\alpha}
  %  \label{eq:10a}
%\end{equation}    
%\begin{equation}
 %       t=l+(r-l)y
  %      \label{eq:10b}
%\end{equation}
%\begin{equation}
 %       h=\min (1, \max (0, t))
  %      \label{eq:10c}
%\end{equation}




%The rectified variable $H\sim \texttt{HardKuma}(\alpha, \beta, l, r)$ is modification of Kumaraswamy distribution. We can get samples from Hardkuma by 
%sampling uniform variable $U\sim \mathcal{U}(0, 1)$ and applying inverse cdf of kuma distribution($Y \sim \texttt{Kuma}(\alpha, \beta)$) over U as eq.(\ref{eq:10a}), then shifting and scaling the result to cover the stretched support (\ref{eq:10b}), and finally, applying the rectifier in order to get a sample in the closed interval [0, 1] (\ref{eq:10c}).
\todo[inline]{h,t,k are not defined. BAsically what I don't understand of fidn confusing is how exactly teh sampling is done. Is it not done using equation 5? where h is your uniform random variable. And what does HardKuma in Equation 6 function corresponds to? For example Y was sampled from Kuma but was never used later.}\mandeep{h and t are defined."k" is replaced by y now. "h" is sample from HardKuma. For Sampling, we explained it in section 3.2 (in form of text only). So, we start with $y\in Kuma(\alpha,\beta)$ and end up with $h\in HardKuma(\alpha,\beta,l,r)$ using the following equations:

\begin{equation}
F_{Y}^{-1}(U ; \alpha, \beta) \sim \operatorname{Kuma}(\alpha, \beta)
\label{eq:10}
\end{equation}

\begin{equation}
    y=F_{Y}^{-1}(u ; \alpha, \beta)=\left(1-(1-u)^{1 / \beta}\right)^{1/\alpha}
    \label{eq:10a}
\end{equation}    
\begin{equation}
        t=l+(r-l)y
        \label{eq:10b}
\end{equation}
\begin{equation}
        h=\min (1, \max (0, t))
        \label{eq:10c}
\end{equation}

We can add these equations too. 
}

\todo[inline]{I would suggest taht we should keep in teh main paper the computation of your variable $z_{ij}$ given uniform variable u and your other apramters $\alpha$ and $\beta$. REst can go to supplementary material}
\thorben{How about directly writing $z = ....$ and on the left side only use u which comes from uniform. It should be feasible to combine eq. 8-10 into one line. It should be
$$
z=\min (1, \max (0, l+(r-l)\left(1-(1-u)^{1 / \beta}\right)^{1/\alpha}))
$$
}

\mandeep{Acc to me, reader we confuse while getting partial derivatives. By equations, it is very easy to understand the derivatives}


For the training, we need the gradient with respect to uniform variable $u$. Let $\mathcal{L}(u)$ be the function of uniform variable \textit{u}.
The gradient of the function $\mathcal{L}(u)$ with respect to  $u$ can be computed by applying the chain rule. For details we refer to \cite{bastings2019interpretable}. 

% $$
%\frac{\partial \mathcal{L}}{\partial u}=\frac{\partial \mathcal{L}}{\partial h} \times \frac{\partial h}{\partial t} \times \frac{\partial t}{\partial y} \times \frac{\partial y}{\partial u}
% $$
%by chain rule, the eq.(\ref{eq:10a}) and eq.(\ref{eq:10b}) have well defined partial derivatives. 
%Also the eq.(\ref{eq:10c}) has well defined of h w.r.t. t when $t<0$, $t>1$ and $0<t<1$. But the derivative is not defined for $t \in\{0,1\}$, which is a finite set with 0 measure and hence we say this reparameterisation is differentiable \textit{almost everywhere}.





%So, the partial derivative of the function 
%$\mathcal{L}(u)$ is calculated as:

% $$
% \frac{\partial \mathcal{L}}{\partial u}=\frac{\partial \mathcal{L}}{\partial h} \times \frac{\partial h}{\partial t} \times \frac{\partial t}{\partial y} \times \frac{\partial y}{\partial u}
% $$
%by chain rule. The term $\frac{\partial \mathcal{L}}{\partial h}$ depends on a differentiable observation model and has a well defined derivative. Also, the term $\frac{\partial h}{\partial t}$ is the derivative of the hard-sigmoid i.e. $h = \texttt{min}(1, \texttt{max}(0, t))$ function, which is 0 for $t<0$ or $t>1,1$ for $0 \leq t<1,$ and not defined for $t \in\{0,1\}$. The term $\frac{\partial t}{\partial k}=r-l$ follows directly from eq.( \ref{eq:10b}) the term $\frac{\partial k}{\partial u}=\frac{\partial}{\partial u} F_{K}^{-1}(u ; a, b)$ depends on the
%Kumaraswamy inverse cdf eq.(\ref{eq:10a}) and has well defined derivative. Thus the only two discontinuities happen for $t \in\{0,1\},$ which is a finite set with 0 measure under the stretched Kumaraswamy and hence we say this reparameterisation is differentiable almost everywhere.








==> introduction.tex <==

\section{Introduction}
\label{sec:intro}

%
Graph neural networks (GNNs) are a powerful family of models that operate over graph-structured data and have achieved state-of-the-art performance on node and graph classification tasks. 
GNNs aggregate node feature information using the input graph structure as inductive biases resulting in flexible and powerful learning models.
Although expressive and flexible, current GNNs lack interpretability and limited attention has been paid to building interpretable GNNs in general. 
Existing approaches for building explainable GNNs tend to focus on \textit{post-hoc interpretability}, i.e., they attempt to explain predictions of a GNN mode after the model has been trained~\cite{funke2021zorro,ying2019:gnnexplainer,XGNN2020}.
However, a fundamental limitation of such post-hoc approaches is that explanations might not necessarily be accurate reflections of the model decisions~\cite{rudin2019stop}. 
Second, and more worrisome, is the problem of the evaluation of interpretability techniques due to the difficulty in gathering ground truth for evaluating an explanation~\cite{lage2019evaluation,zhang2019dissonance}.
%
Consequently, it is unclear if the model or the explanation is inaccurate for a given decision.

%
An alternate design methodology is to ensure \textit{interpretability by design} by explicitly inducing \emph{sparsification} into GNN models.
Sparsification in this context refers to selecting a subset of neighborhood nodes (for a given query node) that are employed during the aggregation operation. 
There are two major benefits for explicit sparsification in GNNs.
First, explicit sparsification is sometimes necessary in real-world graphs that might contain task-irrelevant edges. 
Hence, a lack of explicit sparsification in GNNs models might result in the aggregation of unnecessary neighborhood information and degrade generalization. 
Secondly, as we show in this work, sparsification also helps to overcome the issue of \emph{over-smoothing}~\cite{li2018deeper} in deep GNNs.
\begin{figure}
  \centering
  \includegraphics[width=.9\textwidth]{Figures/kedge-sparsification.pdf}
  \caption{
  Given feature vectors of query node and its neighbor, \approach{} learns \hardkuma{} distributions for each edge in the original graph. Hence, we learn which edges can be masked without affecting performance.}
  \label{fig:1}
\end{figure}
In this work, we develop a plug-and-play \emph{interpretable by design} approach, which can be incorporated into any GNN model. 
Our approach, which we refer to as \approach{}, learns to actively sparsify the input graph towards improving model interpretability by learning to drop task-irrelevant edges.
Specifically, we build an \emph{adjacency matrix generator} layer, which is given as input the query node and its neighborhood, that selects the most important neighbors (see Figure~\ref{fig:1}), which are then used as input to the GNN layer. 
We model our neighborhood mask using the \hardkuma{} distribution~\cite{kumaraswamy1980generalized}, which exhibits a mix of discrete and continuous behavior. 
We take advantage of this particular property of \hardkuma{} distribution to achieve binary selections and gradient-based training at the same time. 
Our generator layer can be plugged either before the GNN layers or after each GNN layer giving rise to \approach{} and \approach{}-layerwise variants, respectively. 
In particular, the learned neighborhood is layer-dependent in the case of the \approach{}-layerwise variant. Intuitively, each GNN layer learns different properties of a node and might be dependent on different neighborhoods in each layer.

We demonstrate the effectiveness of \approach{} by extensive experimentation on three well-known citation networks and three state-of-the-art GNN models.
We show that \approach{} can remove a significant proportion of edges without compromising performance. 
We observe that the combination of the GNN model and dataset properties, greatly influences the ratio of removed edges by \approach{}. 
In particular, \approach{} removes $83\%$ of the edges on PubMed when using Simple Graph Convolution (SGC).
Moreover, we observe that the effect of over-smoothing on deep GNNs is significantly reduced by \approach{}-layerwise which induces a layer-specific sparser neighborhood. 

%
\subsection{Summary of contributions}

To summarize, we make the following contributions.
\begin{enumerate}
    \item We develop \approach{} which is based on principles of achieving interpretability via input sparsity. \approach{} is easy to incorporate into any existing GNN architecture.
    \item We develop an end-to-end trainable framework achieving binary selection and gradient-based optimization at the same time.
    \item We showcase the superiority of our approach by extensive experiments on three benchmark datasets. 
    In particular, we demonstrate our approach's effectiveness in pruning a high percentage of node neighborhoods without compromising performance.
\end{enumerate}

